Prospects for probing dark matter with filamentary 21cm emission

The cosmic web contains most of the matter in the Universe, and its filamentary structure is closely related to the properties of dark matter. Compared with the cold dark matter (CDM) model, warm dark matter (WDM) suppresses the formation of low-mass halos and produces smoother cosmic filaments. In this work, we explore whether filamentary 21cm emission can be used to distinguish between these two dark matter models at $z=4$ and $2.5$. We generate intrinsic 21cm brightness temperature maps from cosmological hydrodynamical simulations and produce mock observations by convolving them with Gaussian beams of different angular resolutions. We then compare the predicted filament signals with the expected sensitivities of SKA1-Low and SKA2-Low. We find that the intrinsic 21cm emission clearly reflects the different filament morphologies in the CDM and WDM models, particularly at $z=4$. However, these differences rapidly disappear as the beam size increases, especially for beam sizes larger than 6 arcsec. Although larger beams improve the observational sensitivity, they also erase the small-scale structures that encode the dark matter information. As a result, neither SKA1-Low nor the planned SKA2-Low can directly resolve individual filaments with sufficient sensitivity to distinguish between the two models. We therefore conclude that direct imaging of cosmic filaments and constraining dark matter through their morphology are unlikely to be feasible with current and planned SKA-Low facilities.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

